A Theory for Colors of Strongly Correlated Electronic Systems

Many strongly correlated transition metal insulators are colored, even though they have large fundamental band gaps and no quasi-particle excitations in the visible range. Why such insulators possess the colors they do poses a serious challenge for any many-body theory to reliably pick up the interactions responsible for the color. We pick two archetypal cases as examples: NiO with green color and MnF\textsubscript{2} with pink color. The body of literature around the collective charge transitions (excitons) that are responsible for the color in these and other strongly correlated systems, often fail to disentangle two important factors: what makes them form and what makes them optically bright. An adequate answer requires a theoretical approach able to compute such excitations in periodic crystals, reliably and without free parameters -- a formidable challenge. We employ two kinds of advanced \emph{ab initio} many body Green's function theories to investigate both optical and spin susceptibilities. The first, a perturbative theory based on low-order extensions of the $GW$ approximation, is able to explain the color in NiO, and indeed well describe the dielectric response over the entire frequency spectrum, while the same theory is unable to explain why MnF\textsubscript{2} is pink. We show its color originates from higher order spin-flip transitions that modify the optical response. This phenomenon is not captured by low-order perturbation theory, but it is contained in dynamical mean-field theory (DMFT), which has a dynamical spin-flip vertex that contributes to the charge susceptibility. We show that symmetry lowering mechanisms, such as spin-orbit coupling, odd-parity phonons and Jan-Teller distortions, determine how `bright' these excitons are, but are not fundamental to their existence.

==> words <==
Many strongly correlated transition metal insulators are colored, even though they have large fundamental band gaps and no quasi-particle excitations in the visible range. Why such insulators possess the colors they do poses a serious challenge for any many-body theory to reliably pick up the interactions responsible for the color.  We pick two archetypal cases as examples: NiO with green color and MnF\textsubscript{2} with pink color.  The body of literature around the collective charge transitions (excitons) that are responsible for the color in these and other strongly correlated systems, often fail to disentangle two important factors: what makes them form and what makes them optically bright. An adequate answer requires a theoretical approach able to compute such excitations in periodic crystals, reliably and without free parameters---a formidable challenge. We employ two kinds of advanced \emph{ab initio} many body Green's function theories to investigate both optical and spin susceptibilities.  The first, a perturbative theory based on low-order extensions of the $GW$ approximation, is able to explain the color in NiO, and indeed well describe the dielectric response over the entire frequency spectrum, while the same theory is unable to explain why MnF\textsubscript{2} is pink.  We show its color originates from higher order spin-flip transitions that modify the optical response.  This phenomenon is not captured by low-order perturbation theory, but it is contained in dynamical mean-field theory (DMFT), which has a dynamical spin-flip vertex that contributes to the charge susceptibility.  We show that symmetry lowering mechanisms, such as spin-orbit coupling, odd-parity phonons and Jan-Teller distortions, determine how `bright' these excitons are, but are not fundamental to their existence. 

